A Puzzle-Based Dataset for Natural Language Inference

We provide here a dataset for tasks related to natural language understanding and natural language inference. The dataset contains logical puzzles in natural language from three domains: comparing puzzles, knighs and knaves, and zebra puzzles. Each puzzle is associated with the entire set of atomic questions that can be generated based on the relations and individuals occurring in the text. For each question we provide the correct answer: entailment, contradiction or ambiguity. The answer's correctness is verified against theorem provers. Good puzzles have two properties: (i) each piece of information is necessary and (ii) no unnecessary information is provided. These properties make puzzles interesting candidates for machine comprehension tasks.

==> A Puzzle-based dataset for Natural Language Inference/bg.tex <==
   (shorter(x,y) & shorter(y,z) -> shorter(x,z)).           %transitivity
   (taller(x,y)  & taller(y,z)  -> taller(x,z)).
   exists x (tallest(x) & (all y (tallest(y) -> y=x))).
   exists x (shortest(x) & (all y ((shortest(y) -> x=y)))).
   all x all y (taller(x,y) & taller(y,x) -> x=y).          %antisymmetry
   all x all y (shorter(x,y) & shorter(y,x) -> x=y).
  -taller(x,x & -shorter(x,x).                              %irreflexivity
   all x all y (shorter(x,y) | x=y | taller(x,y)).          %trichotomy
   (shorter(x,y) -> (x!=y & -taller(x,y))).
   (x=y) -> (-shorter(x,y) & -taller(x,y)).
   (taller(x,y) -> (x!=y & -shorter(x,y))).
   exists x (all y (-shorter(y,x)) & shortest(x)). 
   exists x (all y (-taller(y,x)) & tallest(x)). 
   taller(x,y) <-> shorter(y,x). 

==> A Puzzle-based dataset for Natural Language Inference/grammar.tex <==
#Grammar Rules

S[SEM = <?subj(?vp)>] -> NP[NUM=?n,SEM=?subj] VP[NUM=?n,SEM=?vp]
NP[LOC=?l,NUM=?n,SEM=?np] -> PropN[LOC=?l,NUM=?n,SEM=?np] | InterPron[LOC=?l,NUM=?n,SEM=?np] | Nom[NUM=?n,SEM=?np] 
NP[+COP, NUM=?n, SEM=?nom ] -> Det[NUM=?n] Nom[NUM=?n, SEM=?nom]
NP[NUM=?n, SEM=<?det(?adj, ?nom)>] -> Det[NUM=sg, SEM=?det] Adj[GRD=?abs, SEM=?adj] Nom[NUM=sg,SEM=?nom] 
VP[NUM=?n,SEM=<?v(?prd)>] -> AuxP[+COP,NUM=?n,SEM=?v] Pred[SEM=?prd]
VP[NUM=?n,SEM=<?cc(?prd1, ?prd2)>] -> VP[NUM=?n,SEM=?prd1] CC[BOUND=?vpToVp, SEM=?cc] VP[NUM=?n,SEM=?prd2]
VP[NUM=?n,SEM=<?cc(?prd1, ?prd2)>] -> VP[NUM=?n,SEM=?prd1] CC[BOUND=?vpToVp, SEM=?cc] AdjP[GRD=?rel, SEM=?prd2]
AdjP[GRD=?rel, SEM=<?quant(?adj(?pp))>] -> Quantifier[SEM=?quant] Adj[GRD=?rel, SEM=?adj] PP[+than,SEM=?pp]
AdjP[GRD=?rel, SEM=<?adj(?pp)>] -> Adj[GRD=?rel, SEM=?adj] PP[+than,SEM=?pp]
AdjP[GRD=?rel, SEM=<?neg(?adj, ?pp)>] ->  Neg[SEM=?neg] Adj[GRD=?rel, SEM=?adj] PP[+than,SEM=?pp]
AdjP[GRD=?abs, SEM=<?adj>] -> Det[NUM=sg] Adj[GRD=?abs, SEM=?adj] 
PP[+than, SEM=?np] -> P[+than] NP[SEM=?np]
AuxP[COP=?c,NUM=?n,SEM=<?neg(?aux)>] -> Aux[COP=?c,NUM=?n,SEM=?aux] Neg[SEM=?neg]
....
#Lexical Rules
PropN[-LOC,NUM=sg,SEM=<\P.P(Mike)>] -> 'Mike'
PropN[-LOC,NUM=sg,SEM=<\P.P(Sally)>] -> 'Sally'
PropN[-LOC,NUM=sg,SEM=<\P.P(Katy)>] -> 'Katy' 
PropN[-LOC,NUM=sg,SEM=<\P.P(Ted)>] -> 'Ted'
PropN[-LOC,NUM=sg,SEM=<\P.P(Bob)>] -> 'Bob'
Det[NUM=sg,SEM=<\P Q x.(P(x) & Q(x))>] -> 'the'
InterPron[-LOC, NUM=sg, SEM=<\P.P(x)>] -> 'who' | 'Who'
RelPron[SEM=<\Q x P.((P(x) & Q(x)))>] -> 'who'
Aux[+COP,NUM=sg,SEM=<\P x.P(x)>,tns=pres] -> 'is' | 'Is'
Aux[+COP,NUM=,SEM=<\P x.P(x)>,tns=pres] -> 'are' | 'Are'
CC[BOUND=?vpToVp, SEM=<\P Q x.((P(x) & Q(x)))>] -> 'but'
Adj[GRD=rel, SEM=<\X x.X(\y.(taller(x,y)))>] -> 'taller'
Adj[GRD=rel, SEM=<\X x.X(\y.(shorter(x,y)))>] -> 'shorter'
Adj[GRD=abs, SEM=<\x.(shortest(x))>] -> 'shortest'
Adj[GRD=abs, SEM=<\x.(tallest(x))>] -> 'tallest'
Quantifier[SEM=<\P. P>] -> 'little'
Quantifier[SEM=<\P. P>] -> 'too'
Question[] -> '?'
...

Knight knaves Grammar

#Grammar rules
S[SEM=<?np(?vp)>] -> NP[NUM=?n, SEM=?np] VP[NUM=?n, SEM=?vp]
S[SEM=?vp] -> Pron[NUM=?n] VP[NUM=?n2, SEM=?vp]
S[SEM=<?that(?sent1, ?sent2)>] -> S[SEM=?sent1] Conj[BOUND=sentences, TYPE=thatClause, SEM=?that] CompoundSent[SEM=?sent2]
CompoundSent[SEM=<?conjEither(?sent1, ?sent2)>] -> Conj[+either,SEM=?conjEither] S[SEM=?sent1] Conj[BOUND=sentences, SEM=?conj2] S[SEM=?sent2]
CompoundSent[SEM=<?conj2(?sent1, ?sent2)>] -> Quantifier[+BOTH] S[SEM=?sent1] Conj[BOUND=sentences, SEM=?conj2] S[SEM=?sent2]
PP[TYPE=?type] -> P[+on] NP[TYPE=?type, NUM=?n]
NP[TYPE=where, NUM=?n] -> Det[SEM=?det] Nom[NUM=?n, SEM=?nom]
NP[NUM=?n, SEM=?nom] -> Nom[NUM=?n, SEM=?nom]
NP[LOC=?l,NUM=?n,SEM=?np] -> PropN[LOC=?l,NUM=?n,SEM=?np] 
NP[NUM=?n, SEM=?nom] -> Numeral[NUM=?n] Nom[NUM=?n, SEM=?nom]
VP[NUM=?n,SEM=<?v(?prd)>, TYPE=one] -> AuxP[COP=?c,NUM=?n,SEM=?v, TYPE=one] Pred[SEM=?prd]
VP[NUM=?n,SEM=?vp] -> SV[NUM=?n, SEM=?vp]  
VP[NUM=?n,SEM=?vp] -> Modal[] SV[NUM=?n, SEM=?vp]
VP[NUM=?n,SEM=?vp] -> Modal[] SV[NUM=?n, SEM=?vp] Pron[NUM=sg]
VP[NUM=?n,SEM=?vp] -> SV[NUM=?n, SEM=?vp] Pron[SEM=?pron]
....
#Lexical Rules
PropN[-LOC,NUM=sg,SEM=<\P.P(Sue)>] -> 'Carl'
PropN[-LOC,NUM=sg,SEM=<\P.P(Dave)>] -> 'Dave'
PropN[-LOC,NUM=sg,SEM=<\P.P(Rex)>] -> 'Rex'
PropN[-LOC,NUM=sg,SEM=<\P.P(Bart)>] -> 'Bart'
N[NUM=sg,SEM=<\x.island(x)>] -> 'island'
N[NUM=sg,SEM=<\x.inhabitant(x)>] -> 'inhabitant'
N[NUM=pl,SEM=<\x.inhabitant(x)>] -> 'inhabitants'
N[NUM=sg,SEM=<\x.knight(x)>] -> 'knight'
N[NUM=pl,SEM=<\x.knight(x)>] -> 'knights'
N[NUM=sg,SEM=<\x.knave(x)>] -> 'knave'
N[NUM=pl,SEM=<\x.knave(x)>] -> 'knaves'
Conj[+either, SEM=<\P Q ((P & -Q) | (-P & Q))>] -> 'either'
Conj[BOUND=NP, SEM=<\P Q x.((P(x) | Q(x)))>] -> 'or'
Conj[BOUND=NP, SEM=<\P Q X.((P(X) & Q(X)))>] -> 'and'
Aux[COP=true,NUM=sg,SEM=<\P x.P(x)>,tns=pres] -> 'is'
SV[NUM=sg, PERS=third, SEM=<\x.m(x)>] -> 'says'
SV[NUM=sg, PERS=noThird, SEM=<\x.m(x)>] -> 'say'
Quantifier[+BOTH] -> 'both'
InterPron[-LOC, NUM=sg, SEM=<\P.P(x)>] -> 'who' | 'Who'
Pron[NUM=sg, PERS=third ,SEM=<\P.P(he)>] -> 'he' | 'He'
Modal[] -> 'would' | 'could'
Numeral[NUM=pl] -> 'four'
.......

==> A Puzzle-based dataset for Natural Language Inference/kk.tex <==
formulas(assumptions).
  all x (inhabitant(x) -> knight(x) | knave(x)). 
  all x ((knight(x) -> -knave(x)) & (knave(x) -> -knight(x))).
  knight(x) ->  m(x).                      knave(x)  -> -m(x).
   
  inhabitant(Sue) & inhabitant(Bart) & inhabitant(Rex) & inhabitant(Dave).
  m(Bart) <-> (knight(Rex) & knight(Dave)) | (knave(Rex) & knave(Dave)). 
  m(Dave) <->  knave(Sue). 
  m(Rex)  <->  knave(Bart). 
  m(Sue)  <->  knight(Rex) & knave(Dave).
  Sue!=Rex & Sue!=Bart & Sue!=Dave & Rex!=Bart & Rex!=Dave & Bart!=Dave.
end_of_list.

formulas(goals).
  knave(Dave) & knave(Bart) & knight(Sue) & knight(Rex).
end_of_list.

==> A Puzzle-based dataset for Natural Language Inference/knight-knave-mace4_models.tex <==
mace4 -m -1 -n 4 -c -f knight.in | interpformat

=== Mace4 starting on domain size 4. ===

PUZZLE 3:
------ process 41381 exit (all_models) ------
interpretation( 4, [number = 1,seconds = 0], [
    function(bart, [0]),
    function(dave, [1]),
    function(rex, [2]),
    function(sue, [3]),
    relation(inhabitant(_), [1,1,1,1]),
    relation(knave(_), [1,1,0,0]),
    relation(knight(_), [0,0,1,1]),
    relation(m(_), [0,0,1,1])]).

PUZZLE 4:% without   m(Sue) <-> knight(Rex) & knave(Dave).
=== Mace4 starting on domain size 4. ===

------ process 41687 exit (all_models) ------
interpretation( 4, [number = 1,seconds = 0], [
    function(Bart, [0]),
    function(Dave, [1]),
    function(Rex, [2]),
    function(Sue, [3]),
    relation(inhabitant(_), [1,1,1,1]),
    relation(knave(_), [0,1,1,0]),
    relation(knight(_), [1,0,0,1]),
    relation(m(_), [1,0,0,1])]).
interpretation( 4, [number = 2,seconds = 0], [
    function(Bart, [0]),
    function(Dave, [1]),
    function(Rex, [2]),
    function(Sue, [3]),
    relation(inhabitant(_), [1,1,1,1]),
    relation(knave(_), [1,1,0,0]),
    relation(knight(_), [0,0,1,1]),
    relation(m(_), [0,0,1,1])]).


PUZZLE 5: without   %m(Rex) <->  knave(Bart). 
=== Mace4 starting on domain size 4. ===

------ process 41819 exit (all_models) ------
interpretation( 4, [number = 1,seconds = 0], [
    function(Bart, [0]),
    function(Dave, [1]),
    function(Rex, [2]),
    function(Sue, [3]),
    relation(inhabitant(_), [1,1,1,1]),
    relation(knave(_), [0,0,0,1]),
    relation(knight(_), [1,1,1,0]),
    relation(m(_), [1,1,1,0])]).
interpretation( 4, [number = 2,seconds = 0], [
    function(Bart, [0]),
    function(Dave, [1]),
    function(Rex, [2]),
    function(Sue, [3]),
    relation(inhabitant(_), [1,1,1,1]),
    relation(knave(_), [1,0,1,1]),
    relation(knight(_), [0,1,0,0]),
    relation(m(_), [0,1,0,0])]).
interpretation( 4, [number = 3,seconds = 0], [
    function(Bart, [0]),
    function(Dave, [1]),
    function(Rex, [2]),
    function(Sue, [3]),
    relation(inhabitant(_), [1,1,1,1]),
    relation(knave(_), [1,1,0,0]),
    relation(knight(_), [0,0,1,1]),
    relation(m(_), [0,0,1,1])]).


==> A Puzzle-based dataset for Natural Language Inference/mace4_models_comparison.tex <==
interpretation( 5, [number = 1,seconds = 0], [
    function(Bob, [2]),
    function(Katy, [3]),
    function(Mike, [4]),
    function(Sally, [0]),
    function(Ted, [1]),
    function(c1, [3]),
    function(c2, [2]),
    function(c3, [2]),
    function(c4, [3]),
    relation(shortest(_), [0,0,1,0,0]),
    relation(tallest(_), [0,0,0,1,0]),
    relation(shorter(_,_), [
        0,0,0,1,1,
        1,0,0,1,1,
        1,1,0,1,1,
        0,0,0,0,0,
        0,0,0,1,0]),
    relation(taller(_,_), [
        0,1,1,0,0,
        0,0,1,0,0,
        0,0,0,0,0,
        1,1,1,0,1,
        1,1,1,0,0])]).
interpretation( 5, [number = 2,seconds = 0], [
    function(Bob, [2]),
    function(Katy, [3]),
    function(Mike, [4]),
    function(Sally, [0]),
    function(Ted, [1]),
    function(c1, [4]),
    function(c2, [2]),
    function(c3, [2]),
    function(c4, [4]),
    relation(shortest(_), [0,0,1,0,0]),
    relation(tallest(_), [0,0,0,0,1]),
    relation(shorter(_,_), [
        0,0,0,1,1,
        1,0,0,1,1,
        1,1,0,1,1,
        0,0,0,0,1,
        0,0,0,0,0]),
    relation(taller(_,_), [
        0,1,1,0,0,
        0,0,1,0,0,
        0,0,0,0,0,
        1,1,1,0,0,
        1,1,1,1,0])]).

==> A Puzzle-based dataset for Natural Language Inference/model_zebra_puzzle.tex <==

\begin{table}[H]  \centering % size 5
a: 0 \hspace{.5cm}
b: 1 \hspace{.5cm}
c: 2 \hspace{.5cm}
d: 3 \hspace{.5cm}
e: 4 \hspace{.5cm}
\begin{tabular}{r|rrrrr}
beer: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 1 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
bird: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 1 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
blend: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 1 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
blue: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 1 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
bluemaster: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 1 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
brit: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 1 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
cat: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 1 & 0 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
coffee: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 0 & 1
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
dane: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 1 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
dog: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 1 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
dunhill: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 1 & 0 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
fish: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 0 & 1
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
german: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 0 & 1
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
green: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 0 & 1
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
horse: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 1 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
milk: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 1 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
norwegian: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 1 & 0 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
pallmall: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 1 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
prince: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 0 & 1
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
red: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 1 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
swede: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 1 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
tea: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 1 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
water: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 1 & 0 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
white: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 1 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
yellow: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 1 & 0 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
differentFrom: & 0 & 1 & 2 & 3 & 4\\
\hline
    0 & 0 & 1 & 1 & 1 & 1 \\
    1 & 1 & 0 & 1 & 1 & 1 \\
    2 & 1 & 1 & 0 & 1 & 1 \\
    3 & 1 & 1 & 1 & 0 & 1 \\
    4 & 1 & 1 & 1 & 1 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
neighbor: & 0 & 1 & 2 & 3 & 4\\
\hline
    0 & 0 & 1 & 0 & 0 & 0 \\
    1 & 1 & 0 & 1 & 0 & 0 \\
    2 & 0 & 1 & 0 & 1 & 0 \\
    3 & 0 & 0 & 1 & 0 & 1 \\
    4 & 0 & 0 & 0 & 1 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
rightneighbor: & 0 & 1 & 2 & 3 & 4\\
\hline
    0 & 0 & 1 & 0 & 0 & 0 \\
    1 & 0 & 0 & 1 & 0 & 0 \\
    2 & 0 & 0 & 0 & 1 & 0 \\
    3 & 0 & 0 & 0 & 0 & 1 \\
    4 & 0 & 0 & 0 & 0 & 0
\end{tabular}
\caption{ }
\end{table}

==> A Puzzle-based dataset for Natural Language Inference/name.tex <==

The topic of grey literature deserves more attention, since the quality or trust gap between white and grey literature is smaller and smaller.

In my view, there no enough technical specificity to support follow up. 
The paper can be restricted to at most two pages, maybe a poster.  

Subsection 3.2.4 Analysis the results, though the Results are introduced only in Section 4. 

Which is the relevance of the histogram in Figure 1 for the presentend experiments?
I would refer Figure 2 in the first paragraph of 3.2.3. Document Analysis.

Section 5 - only one subsection 5.1 

Two human agents use four criteria to rate 127 documents.

The study domain (Product managers in software startups) seems to have no impact/relevance on the analysis or method. This suggests that Section 3.1 can be reduced to a single paragraph. 

I see the work presented here as a preliminary analysis, useful to define research questions for the domain of summarisation and gray literature
For instance, the results of RQ3 can be a good starting point for some research questions that require some 


==> A Puzzle-based dataset for Natural Language Inference/zebra.tex <==
formulas(assumptions).
 %a and b are something different 
 differentFrom(a,b).
 differentFrom(a,c).
 differentFrom(a,d).
 differentFrom(a,e).
 differentFrom(b,c).
 differentFrom(b,d).
 differentFrom(b,e).
 differentFrom(c,d).
 differentFrom(c,e).
 differentFrom(d,e).

 %the "differentFrom" relation is symmetrical
 %so we won't bother to write it in both directions
 differentFrom(x,y) ->  differentFrom(y,x).

% Define the "right neighbor" relation among a,b,c,d,e
%b is immediately to the right of a
 rightneighbor(a,b) & rightneighbor(b,c) & rightneighbor(c,d) & rightneighbor(d,e).
 -rightneighbor(a,a) & -rightneighbor(a,c) & -rightneighbor(a,d) & -rightneighbor(a,e).
 -rightneighbor(b,a) & -rightneighbor(b,b) & -rightneighbor(b,d) & -rightneighbor(b,e).
 -rightneighbor(c,a) & -rightneighbor(c,b) & -rightneighbor(c,c) & -rightneighbor(c,e).
 -rightneighbor(d,a) & -rightneighbor(d,b) & -rightneighbor(d,c) & -rightneighbor(d,d).
 -rightneighbor(e,a) & -rightneighbor(e,b) & -rightneighbor(e,c) & -rightneighbor(e,d) & -rightneighbor(e,e).

 % you are the neighbor of someone either if you live just to his right
 % or he lives just to your right (i.e., you live just to his left)
 rightneighbor(x,y) | rightneighbor(y,x) <-> neighbor(x,y).

% Each house has at least one nationality, pet, drink, color, car.

    brit(x) | swede(x) | german(x) | dane(x) | norwegian(x).
    dog(x) | fish(x) | cat(x) | horse(x) | bird(x).
    water(x) | milk(x) | tea(x) | coffee(x) | beer(x).
    pallmall(x) | dunhill(x) | blend(x) | bluemaster(x) | prince(x).
    red(x) | green(x) | blue(x) | yellow(x) | white(x).

% Each property applies to at most one house.

    brit(x) & brit(y) -> -differentFrom(x,y).
    swede(x) & swede(y) -> -differentFrom(x,y).
    german(x) & german(y) -> -differentFrom(x,y).
    dane(x) & dane(y) -> -differentFrom(x,y).
    norwegian(x) & norwegian(y) -> -differentFrom(x,y).
    
    dog(x) & dog(y) -> -differentFrom(x,y).
    bird(x) & bird(y) -> -differentFrom(x,y).
    cat(x) & cat(y) -> -differentFrom(x,y).
    fish(x) & fish(y) -> -differentFrom(x,y).
    horse(x) & horse(y) -> -differentFrom(x,y).
    
    beer(x) & beer(y) -> -differentFrom(x,y).
    milk(x) & milk(y) -> -differentFrom(x,y).
    water(x) & water(y) -> -differentFrom(x,y).
    coffee(x) & coffee(y) -> -differentFrom(x,y).
    tea(x) & tea(y) -> -differentFrom(x,y).
    
    red(x) & red(y) -> -differentFrom(x,y).
    green(x) & green(y) -> -differentFrom(x,y).
    blue(x) & blue(y) -> -differentFrom(x,y).
    yellow(x) & yellow(y) -> -differentFrom(x,y).
    white(x) & white(y) -> -differentFrom(x,y).
    
    pallmall(x) & pallmall(y) -> -differentFrom(x,y).
    dunhill(x) & dunhill(y) -> -differentFrom(x,y).
    blend(x) & blend(y) -> -differentFrom(x,y).
    bluemaster(x) & bluemaster(y) -> -differentFrom(x,y).
    prince(x) & prince(y) -> -differentFrom(x,y).

% The clues.

    brit(x) <-> red(x).
    swede(x) <-> dog(x).
    dane(x) <-> tea(x).
    green(x) & white(y) -> rightneighbor(y,x).
    green(x) <-> coffee(x).
    pallmall(x) <-> bird(x).
    yellow(x) <-> dunhill(x).
    milk(c).
    norwegian(a).    
    blend(x) & cat(y) -> neighbor(x,y).
    horse(x) & dunhill(y) -> neighbor(x,y).
    bluemaster(x) <-> beer(x).    
    german(x) <-> prince(x).
    norwegian(x) & blue(y) -> neighbor(x,y).
    blend(x) & water(y) -> neighbor(x,y).
end_of_list.

==> A Puzzle-based dataset for Natural Language Inference/zebrapuzzle.tex <==
formulas(assumptions).
    differentFrom(x,y) ->  differentFrom(y,x).
    differentFrom(a,b) & differentFrom(a,c) & differentFrom(a,d) & differentFrom(a,e) &  differentFrom(d,e) & differentFrom(b,c) & differentFrom(b,d) ......
    rightneighbor(x,y) | rightneighbor(y,x) <-> neighbor(x,y).
    rightneighbor(a,b) & rightneighbor(b,c) & rightneighbor(c,d) & rightneighbor(d,e).
    -rightneighbor(a,a)  .....
    brit(x) | swede(x) | german(x) | dane(x) | norwegian(x).
    dog(x) | fish(x) | cat(x) | horse(x) | bird(x).
    water(x) | milk(x) | tea(x) | coffee(x) | beer(x).
    pallmall(x) | dunhill(x) | blend(x) | bluemaster(x) | prince(x).
    red(x) | green(x) | blue(x) | yellow(x) | white(x).
    german(x) & german(y) -> -differentFrom(x,y).
    dane(x) & dane(y) -> -differentFrom(x,y).     .....
    dog(x) & dog(y) -> -differentFrom(x,y).   .....
    water(x) & water(y) -> -differentFrom(x,y). .....
    green(x) & green(y) -> -differentFrom(x,y). .....
    dunhill(x) & dunhill(y) -> -differentFrom(x,y). .....
 end_of_list.
brit(x) <-> red(x).                       %the Brit lives in the red house
swede(x) <-> dog(x).                      %the Swede keeps dogs as pets
dane(x) <-> tea(x).                       %the Dane drinks tea
green(x) & white(y) -> rightneighbor(y,x). 
green(x) <-> coffee(x).
pallmall(x) <-> bird(x).
yellow(x) <-> dunhill(x).
milk(c).
norwegian(a).    
blend(x) & cat(y) -> neighbor(x,y).
horse(x) & dunhill(y) -> neighbor(x,y).
bluemaster(x) <-> beer(x).    
german(x) <-> prince(x).               
norwegian(x) & blue(y) -> neighbor(x,y). 
blend(x) & water(y) -> neighbor(x,y).
end_of_list.

==> grammar.tex <==
#Grammar Rules

S[SEM = <?subj(?vp)>] -> NP[NUM=?n,SEM=?subj] VP[NUM=?n,SEM=?vp]
NP[LOC=?l,NUM=?n,SEM=?np] -> PropN[LOC=?l,NUM=?n,SEM=?np] | InterPron[LOC=?l,NUM=?n,SEM=?np] | Nom[NUM=?n,SEM=?np] 
NP[+COP, NUM=?n, SEM=?nom ] -> Det[NUM=?n] Nom[NUM=?n, SEM=?nom]
NP[NUM=?n, SEM=<?det(?adj, ?nom)>] -> Det[NUM=sg, SEM=?det] Adj[GRD=?abs, SEM=?adj] Nom[NUM=sg,SEM=?nom] 
VP[NUM=?n,SEM=<?v(?prd)>] -> AuxP[+COP,NUM=?n,SEM=?v] Pred[SEM=?prd]
VP[NUM=?n,SEM=<?cc(?prd1, ?prd2)>] -> VP[NUM=?n,SEM=?prd1] CC[BOUND=?vpToVp, SEM=?cc] VP[NUM=?n,SEM=?prd2]
VP[NUM=?n,SEM=<?cc(?prd1, ?prd2)>] -> VP[NUM=?n,SEM=?prd1] CC[BOUND=?vpToVp, SEM=?cc] AdjP[GRD=?rel, SEM=?prd2]
AdjP[GRD=?rel, SEM=<?quant(?adj(?pp))>] -> Quantifier[SEM=?quant] Adj[GRD=?rel, SEM=?adj] PP[+than,SEM=?pp]
AdjP[GRD=?rel, SEM=<?adj(?pp)>] -> Adj[GRD=?rel, SEM=?adj] PP[+than,SEM=?pp]
AdjP[GRD=?rel, SEM=<?neg(?adj, ?pp)>] ->  Neg[SEM=?neg] Adj[GRD=?rel, SEM=?adj] PP[+than,SEM=?pp]
AdjP[GRD=?abs, SEM=<?adj>] -> Det[NUM=sg] Adj[GRD=?abs, SEM=?adj] 
PP[+than, SEM=?np] -> P[+than] NP[SEM=?np]
AuxP[COP=?c,NUM=?n,SEM=<?neg(?aux)>] -> Aux[COP=?c,NUM=?n,SEM=?aux] Neg[SEM=?neg]
....
#Lexical Rules
PropN[-LOC,NUM=sg,SEM=<\P.P(Mike)>] -> 'Mike'
PropN[-LOC,NUM=sg,SEM=<\P.P(Sally)>] -> 'Sally'
PropN[-LOC,NUM=sg,SEM=<\P.P(Katy)>] -> 'Katy' 
PropN[-LOC,NUM=sg,SEM=<\P.P(Ted)>] -> 'Ted'
PropN[-LOC,NUM=sg,SEM=<\P.P(Bob)>] -> 'Bob'
Det[NUM=sg,SEM=<\P Q x.(P(x) & Q(x))>] -> 'the'
InterPron[-LOC, NUM=sg, SEM=<\P.P(x)>] -> 'who' | 'Who'
RelPron[SEM=<\Q x P.((P(x) & Q(x)))>] -> 'who'
Aux[+COP,NUM=sg,SEM=<\P x.P(x)>,tns=pres] -> 'is' | 'Is'
Aux[+COP,NUM=,SEM=<\P x.P(x)>,tns=pres] -> 'are' | 'Are'
CC[BOUND=?vpToVp, SEM=<\P Q x.((P(x) & Q(x)))>] -> 'but'
Adj[GRD=rel, SEM=<\X x.X(\y.(taller(x,y)))>] -> 'taller'
Adj[GRD=rel, SEM=<\X x.X(\y.(shorter(x,y)))>] -> 'shorter'
Adj[GRD=abs, SEM=<\x.(shortest(x))>] -> 'shortest'
Adj[GRD=abs, SEM=<\x.(tallest(x))>] -> 'tallest'
Quantifier[SEM=<\P. P>] -> 'little'
Quantifier[SEM=<\P. P>] -> 'too'
Question[] -> '?'
...

Knight knaves Grammar

#Grammar rules
S[SEM=<?np(?vp)>] -> NP[NUM=?n, SEM=?np] VP[NUM=?n, SEM=?vp]
S[SEM=?vp] -> Pron[NUM=?n] VP[NUM=?n2, SEM=?vp]
S[SEM=<?that(?sent1, ?sent2)>] -> S[SEM=?sent1] Conj[BOUND=sentences, TYPE=thatClause, SEM=?that] CompoundSent[SEM=?sent2]
CompoundSent[SEM=<?conjEither(?sent1, ?sent2)>] -> Conj[+either,SEM=?conjEither] S[SEM=?sent1] Conj[BOUND=sentences, SEM=?conj2] S[SEM=?sent2]
CompoundSent[SEM=<?conj2(?sent1, ?sent2)>] -> Quantifier[+BOTH] S[SEM=?sent1] Conj[BOUND=sentences, SEM=?conj2] S[SEM=?sent2]
PP[TYPE=?type] -> P[+on] NP[TYPE=?type, NUM=?n]
NP[TYPE=where, NUM=?n] -> Det[SEM=?det] Nom[NUM=?n, SEM=?nom]
NP[NUM=?n, SEM=?nom] -> Nom[NUM=?n, SEM=?nom]
NP[LOC=?l,NUM=?n,SEM=?np] -> PropN[LOC=?l,NUM=?n,SEM=?np] 
NP[NUM=?n, SEM=?nom] -> Numeral[NUM=?n] Nom[NUM=?n, SEM=?nom]
VP[NUM=?n,SEM=<?v(?prd)>, TYPE=one] -> AuxP[COP=?c,NUM=?n,SEM=?v, TYPE=one] Pred[SEM=?prd]
VP[NUM=?n,SEM=?vp] -> SV[NUM=?n, SEM=?vp]  
VP[NUM=?n,SEM=?vp] -> Modal[] SV[NUM=?n, SEM=?vp]
VP[NUM=?n,SEM=?vp] -> Modal[] SV[NUM=?n, SEM=?vp] Pron[NUM=sg]
VP[NUM=?n,SEM=?vp] -> SV[NUM=?n, SEM=?vp] Pron[SEM=?pron]
....
#Lexical Rules
PropN[-LOC,NUM=sg,SEM=<\P.P(Sue)>] -> 'Carl'
PropN[-LOC,NUM=sg,SEM=<\P.P(Dave)>] -> 'Dave'
PropN[-LOC,NUM=sg,SEM=<\P.P(Rex)>] -> 'Rex'
PropN[-LOC,NUM=sg,SEM=<\P.P(Bart)>] -> 'Bart'
N[NUM=sg,SEM=<\x.island(x)>] -> 'island'
N[NUM=sg,SEM=<\x.inhabitant(x)>] -> 'inhabitant'
N[NUM=pl,SEM=<\x.inhabitant(x)>] -> 'inhabitants'
N[NUM=sg,SEM=<\x.knight(x)>] -> 'knight'
N[NUM=pl,SEM=<\x.knight(x)>] -> 'knights'
N[NUM=sg,SEM=<\x.knave(x)>] -> 'knave'
N[NUM=pl,SEM=<\x.knave(x)>] -> 'knaves'
Conj[+either, SEM=<\P Q ((P & -Q) | (-P & Q))>] -> 'either'
Conj[BOUND=NP, SEM=<\P Q x.((P(x) | Q(x)))>] -> 'or'
Conj[BOUND=NP, SEM=<\P Q X.((P(X) & Q(X)))>] -> 'and'
Aux[COP=true,NUM=sg,SEM=<\P x.P(x)>,tns=pres] -> 'is'
SV[NUM=sg, PERS=third, SEM=<\x.m(x)>] -> 'says'
SV[NUM=sg, PERS=noThird, SEM=<\x.m(x)>] -> 'say'
Quantifier[+BOTH] -> 'both'
InterPron[-LOC, NUM=sg, SEM=<\P.P(x)>] -> 'who' | 'Who'
Pron[NUM=sg, PERS=third ,SEM=<\P.P(he)>] -> 'he' | 'He'
Modal[] -> 'would' | 'could'
Numeral[NUM=pl] -> 'four'
.......

==> kk.tex <==
formulas(assumptions).
  all x (inhabitant(x) -> knight(x) | knave(x)). 
  all x ((knight(x) -> -knave(x)) & (knave(x) -> -knight(x))).
  knight(x) ->  m(x).                      knave(x)  -> -m(x).
   
  inhabitant(Sue) & inhabitant(Bart) & inhabitant(Rex) & inhabitant(Dave).
  m(Bart) <-> (knight(Rex) & knight(Dave)) | (knave(Rex) & knave(Dave)). 
  m(Dave) <->  knave(Sue). 
  m(Rex)  <->  knave(Bart). 
  m(Sue)  <->  knight(Rex) & knave(Dave).
  Sue!=Rex & Sue!=Bart & Sue!=Dave & Rex!=Bart & Rex!=Dave & Bart!=Dave.
end_of_list.

formulas(goals).
  knave(Dave) & knave(Bart) & knight(Sue) & knight(Rex).
end_of_list.

==> knight-knave-mace4_models.tex <==
mace4 -m -1 -n 4 -c -f knight.in | interpformat

=== Mace4 starting on domain size 4. ===

PUZZLE 3:
------ process 41381 exit (all_models) ------
interpretation( 4, [number = 1,seconds = 0], [
    function(bart, [0]),
    function(dave, [1]),
    function(rex, [2]),
    function(sue, [3]),
    relation(inhabitant(_), [1,1,1,1]),
    relation(knave(_), [1,1,0,0]),
    relation(knight(_), [0,0,1,1]),
    relation(m(_), [0,0,1,1])]).

PUZZLE 4:% without   m(Sue) <-> knight(Rex) & knave(Dave).
=== Mace4 starting on domain size 4. ===

------ process 41687 exit (all_models) ------
interpretation( 4, [number = 1,seconds = 0], [
    function(Bart, [0]),
    function(Dave, [1]),
    function(Rex, [2]),
    function(Sue, [3]),
    relation(inhabitant(_), [1,1,1,1]),
    relation(knave(_), [0,1,1,0]),
    relation(knight(_), [1,0,0,1]),
    relation(m(_), [1,0,0,1])]).
interpretation( 4, [number = 2,seconds = 0], [
    function(Bart, [0]),
    function(Dave, [1]),
    function(Rex, [2]),
    function(Sue, [3]),
    relation(inhabitant(_), [1,1,1,1]),
    relation(knave(_), [1,1,0,0]),
    relation(knight(_), [0,0,1,1]),
    relation(m(_), [0,0,1,1])]).


PUZZLE 5: without   %m(Rex) <->  knave(Bart). 
=== Mace4 starting on domain size 4. ===

------ process 41819 exit (all_models) ------
interpretation( 4, [number = 1,seconds = 0], [
    function(Bart, [0]),
    function(Dave, [1]),
    function(Rex, [2]),
    function(Sue, [3]),
    relation(inhabitant(_), [1,1,1,1]),
    relation(knave(_), [0,0,0,1]),
    relation(knight(_), [1,1,1,0]),
    relation(m(_), [1,1,1,0])]).
interpretation( 4, [number = 2,seconds = 0], [
    function(Bart, [0]),
    function(Dave, [1]),
    function(Rex, [2]),
    function(Sue, [3]),
    relation(inhabitant(_), [1,1,1,1]),
    relation(knave(_), [1,0,1,1]),
    relation(knight(_), [0,1,0,0]),
    relation(m(_), [0,1,0,0])]).
interpretation( 4, [number = 3,seconds = 0], [
    function(Bart, [0]),
    function(Dave, [1]),
    function(Rex, [2]),
    function(Sue, [3]),
    relation(inhabitant(_), [1,1,1,1]),
    relation(knave(_), [1,1,0,0]),
    relation(knight(_), [0,0,1,1]),
    relation(m(_), [0,0,1,1])]).


==> mace4_models_comparison.tex <==
interpretation( 5, [number = 1,seconds = 0], [
    function(Bob, [2]),
    function(Katy, [3]),
    function(Mike, [4]),
    function(Sally, [0]),
    function(Ted, [1]),
    function(c1, [3]),
    function(c2, [2]),
    function(c3, [2]),
    function(c4, [3]),
    relation(shortest(_), [0,0,1,0,0]),
    relation(tallest(_), [0,0,0,1,0]),
    relation(shorter(_,_), [
        0,0,0,1,1,
        1,0,0,1,1,
        1,1,0,1,1,
        0,0,0,0,0,
        0,0,0,1,0]),
    relation(taller(_,_), [
        0,1,1,0,0,
        0,0,1,0,0,
        0,0,0,0,0,
        1,1,1,0,1,
        1,1,1,0,0])]).
interpretation( 5, [number = 2,seconds = 0], [
    function(Bob, [2]),
    function(Katy, [3]),
    function(Mike, [4]),
    function(Sally, [0]),
    function(Ted, [1]),
    function(c1, [4]),
    function(c2, [2]),
    function(c3, [2]),
    function(c4, [4]),
    relation(shortest(_), [0,0,1,0,0]),
    relation(tallest(_), [0,0,0,0,1]),
    relation(shorter(_,_), [
        0,0,0,1,1,
        1,0,0,1,1,
        1,1,0,1,1,
        0,0,0,0,1,
        0,0,0,0,0]),
    relation(taller(_,_), [
        0,1,1,0,0,
        0,0,1,0,0,
        0,0,0,0,0,
        1,1,1,0,0,
        1,1,1,1,0])]).

==> model_zebra_puzzle.tex <==

\begin{table}[H]  \centering % size 5
a: 0 \hspace{.5cm}
b: 1 \hspace{.5cm}
c: 2 \hspace{.5cm}
d: 3 \hspace{.5cm}
e: 4 \hspace{.5cm}
\begin{tabular}{r|rrrrr}
beer: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 1 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
bird: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 1 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
blend: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 1 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
blue: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 1 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
bluemaster: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 1 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
brit: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 1 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
cat: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 1 & 0 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
coffee: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 0 & 1
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
dane: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 1 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
dog: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 1 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
dunhill: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 1 & 0 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
fish: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 0 & 1
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
german: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 0 & 1
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
green: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 0 & 1
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
horse: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 1 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
milk: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 1 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
norwegian: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 1 & 0 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
pallmall: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 1 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
prince: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 0 & 1
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
red: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 1 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
swede: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 1 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
tea: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 1 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
water: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 1 & 0 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
white: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 0 & 0 & 0 & 1 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
yellow: & 0 & 1 & 2 & 3 & 4\\
\hline
   & 1 & 0 & 0 & 0 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
differentFrom: & 0 & 1 & 2 & 3 & 4\\
\hline
    0 & 0 & 1 & 1 & 1 & 1 \\
    1 & 1 & 0 & 1 & 1 & 1 \\
    2 & 1 & 1 & 0 & 1 & 1 \\
    3 & 1 & 1 & 1 & 0 & 1 \\
    4 & 1 & 1 & 1 & 1 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
neighbor: & 0 & 1 & 2 & 3 & 4\\
\hline
    0 & 0 & 1 & 0 & 0 & 0 \\
    1 & 1 & 0 & 1 & 0 & 0 \\
    2 & 0 & 1 & 0 & 1 & 0 \\
    3 & 0 & 0 & 1 & 0 & 1 \\
    4 & 0 & 0 & 0 & 1 & 0
\end{tabular} \hspace{.5cm}
\begin{tabular}{r|rrrrr}
rightneighbor: & 0 & 1 & 2 & 3 & 4\\
\hline
    0 & 0 & 1 & 0 & 0 & 0 \\
    1 & 0 & 0 & 1 & 0 & 0 \\
    2 & 0 & 0 & 0 & 1 & 0 \\
    3 & 0 & 0 & 0 & 0 & 1 \\
    4 & 0 & 0 & 0 & 0 & 0
\end{tabular}
\caption{ }
\end{table}

==> name.tex <==

The topic of grey literature deserves more attention, since the quality or trust gap between white and grey literature is smaller and smaller.

In my view, there no enough technical specificity to support follow up. 
The paper can be restricted to at most two pages, maybe a poster.  

Subsection 3.2.4 Analysis the results, though the Results are introduced only in Section 4. 

Which is the relevance of the histogram in Figure 1 for the presentend experiments?
I would refer Figure 2 in the first paragraph of 3.2.3. Document Analysis.

Section 5 - only one subsection 5.1 

Two human agents use four criteria to rate 127 documents.

The study domain (Product managers in software startups) seems to have no impact/relevance on the analysis or method. This suggests that Section 3.1 can be reduced to a single paragraph. 

I see the work presented here as a preliminary analysis, useful to define research questions for the domain of summarisation and gray literature
For instance, the results of RQ3 can be a good starting point for some research questions that require some 


==> zebra.tex <==
formulas(assumptions).
 %a and b are something different 
 differentFrom(a,b).
 differentFrom(a,c).
 differentFrom(a,d).
 differentFrom(a,e).
 differentFrom(b,c).
 differentFrom(b,d).
 differentFrom(b,e).
 differentFrom(c,d).
 differentFrom(c,e).
 differentFrom(d,e).

 %the "differentFrom" relation is symmetrical
 %so we won't bother to write it in both directions
 differentFrom(x,y) ->  differentFrom(y,x).

% Define the "right neighbor" relation among a,b,c,d,e
%b is immediately to the right of a
 rightneighbor(a,b) & rightneighbor(b,c) & rightneighbor(c,d) & rightneighbor(d,e).
 -rightneighbor(a,a) & -rightneighbor(a,c) & -rightneighbor(a,d) & -rightneighbor(a,e).
 -rightneighbor(b,a) & -rightneighbor(b,b) & -rightneighbor(b,d) & -rightneighbor(b,e).
 -rightneighbor(c,a) & -rightneighbor(c,b) & -rightneighbor(c,c) & -rightneighbor(c,e).
 -rightneighbor(d,a) & -rightneighbor(d,b) & -rightneighbor(d,c) & -rightneighbor(d,d).
 -rightneighbor(e,a) & -rightneighbor(e,b) & -rightneighbor(e,c) & -rightneighbor(e,d) & -rightneighbor(e,e).

 % you are the neighbor of someone either if you live just to his right
 % or he lives just to your right (i.e., you live just to his left)
 rightneighbor(x,y) | rightneighbor(y,x) <-> neighbor(x,y).

% Each house has at least one nationality, pet, drink, color, car.

    brit(x) | swede(x) | german(x) | dane(x) | norwegian(x).
    dog(x) | fish(x) | cat(x) | horse(x) | bird(x).
    water(x) | milk(x) | tea(x) | coffee(x) | beer(x).
    pallmall(x) | dunhill(x) | blend(x) | bluemaster(x) | prince(x).
    red(x) | green(x) | blue(x) | yellow(x) | white(x).

% Each property applies to at most one house.

    brit(x) & brit(y) -> -differentFrom(x,y).
    swede(x) & swede(y) -> -differentFrom(x,y).
    german(x) & german(y) -> -differentFrom(x,y).
    dane(x) & dane(y) -> -differentFrom(x,y).
    norwegian(x) & norwegian(y) -> -differentFrom(x,y).
    
    dog(x) & dog(y) -> -differentFrom(x,y).
    bird(x) & bird(y) -> -differentFrom(x,y).
    cat(x) & cat(y) -> -differentFrom(x,y).
    fish(x) & fish(y) -> -differentFrom(x,y).
    horse(x) & horse(y) -> -differentFrom(x,y).
    
    beer(x) & beer(y) -> -differentFrom(x,y).
    milk(x) & milk(y) -> -differentFrom(x,y).
    water(x) & water(y) -> -differentFrom(x,y).
    coffee(x) & coffee(y) -> -differentFrom(x,y).
    tea(x) & tea(y) -> -differentFrom(x,y).
    
    red(x) & red(y) -> -differentFrom(x,y).
    green(x) & green(y) -> -differentFrom(x,y).
    blue(x) & blue(y) -> -differentFrom(x,y).
    yellow(x) & yellow(y) -> -differentFrom(x,y).
    white(x) & white(y) -> -differentFrom(x,y).
    
    pallmall(x) & pallmall(y) -> -differentFrom(x,y).
    dunhill(x) & dunhill(y) -> -differentFrom(x,y).
    blend(x) & blend(y) -> -differentFrom(x,y).
    bluemaster(x) & bluemaster(y) -> -differentFrom(x,y).
    prince(x) & prince(y) -> -differentFrom(x,y).

% The clues.

    brit(x) <-> red(x).
    swede(x) <-> dog(x).
    dane(x) <-> tea(x).
    green(x) & white(y) -> rightneighbor(y,x).
    green(x) <-> coffee(x).
    pallmall(x) <-> bird(x).
    yellow(x) <-> dunhill(x).
    milk(c).
    norwegian(a).    
    blend(x) & cat(y) -> neighbor(x,y).
    horse(x) & dunhill(y) -> neighbor(x,y).
    bluemaster(x) <-> beer(x).    
    german(x) <-> prince(x).
    norwegian(x) & blue(y) -> neighbor(x,y).
    blend(x) & water(y) -> neighbor(x,y).
end_of_list.

==> zebrapuzzle.tex <==
formulas(assumptions).
    differentFrom(x,y) ->  differentFrom(y,x).
    differentFrom(a,b) & differentFrom(a,c) & differentFrom(a,d) & differentFrom(a,e) &  differentFrom(d,e) & differentFrom(b,c) & differentFrom(b,d) ......
    rightneighbor(x,y) | rightneighbor(y,x) <-> neighbor(x,y).
    rightneighbor(a,b) & rightneighbor(b,c) & rightneighbor(c,d) & rightneighbor(d,e).
    -rightneighbor(a,a)  .....
    brit(x) | swede(x) | german(x) | dane(x) | norwegian(x).
    dog(x) | fish(x) | cat(x) | horse(x) | bird(x).
    water(x) | milk(x) | tea(x) | coffee(x) | beer(x).
    pallmall(x) | dunhill(x) | blend(x) | bluemaster(x) | prince(x).
    red(x) | green(x) | blue(x) | yellow(x) | white(x).
    german(x) & german(y) -> -differentFrom(x,y).
    dane(x) & dane(y) -> -differentFrom(x,y).     .....
    dog(x) & dog(y) -> -differentFrom(x,y).   .....
    water(x) & water(y) -> -differentFrom(x,y). .....
    green(x) & green(y) -> -differentFrom(x,y). .....
    dunhill(x) & dunhill(y) -> -differentFrom(x,y). .....
 end_of_list.
brit(x) <-> red(x).                       %the Brit lives in the red house
swede(x) <-> dog(x).                      %the Swede keeps dogs as pets
dane(x) <-> tea(x).                       %the Dane drinks tea
green(x) & white(y) -> rightneighbor(y,x). 
green(x) <-> coffee(x).
pallmall(x) <-> bird(x).
yellow(x) <-> dunhill(x).
milk(c).
norwegian(a).    
blend(x) & cat(y) -> neighbor(x,y).
horse(x) & dunhill(y) -> neighbor(x,y).
bluemaster(x) <-> beer(x).    
german(x) <-> prince(x).               
norwegian(x) & blue(y) -> neighbor(x,y). 
blend(x) & water(y) -> neighbor(x,y).
end_of_list.
